Learning about social learning in MOOCs: From statistical analysis to generative model

We study user behavior in the courses offered by a major Massive Online Open Course (MOOC) provider during the summer of 2013. Since social learning is a key element of scalable education in MOOCs and is done via online discussion forums, our main focus is in understanding forum activities. Two salient features of MOOC forum activities drive our research: 1. High decline rate: for all courses studied, the volume of discussions in the forum declines continuously throughout the duration of the course. 2. High-volume, noisy discussions: at least 30% of the courses produce new discussion threads at rates that are infeasible for students or teaching staff to read through. Furthermore, a substantial portion of the discussions are not directly course-related. We investigate factors that correlate with the decline of activity in the online discussion forums and find effective strategies to classify threads and rank their relevance. Specifically, we use linear regression models to analyze the time series of the count data for the forum activities and make a number of observations, e.g., the teaching staff's active participation in the discussion increases the discussion volume but does not slow down the decline rate. We then propose a unified generative model for the discussion threads, which allows us both to choose efficient thread classifiers and design an effective algorithm for ranking thread relevance. Our ranking algorithm is further compared against two baseline algorithms, using human evaluation from Amazon Mechanical Turk. The authors on this paper are listed in alphabetical order. For media and press coverage, please refer to us collectively, as "researchers from the EDGE Lab at Princeton University, together with collaborators at Boston University and Microsoft Corporation."

==> a-courses.tex <==
\section{List of courses in our analysis}
Table~\ref{atab:stat} gives the set of courses used in the statistical analysis. 
Table~\ref{atab:shapiro} gives the set of courses whose count difference statistics
passes the Shapiro test (see Section~\ref{sec:prelim}). Table~\ref{atab:forum} shows the list of courses
in the generative model analysis and its applications (Section~\ref{sec:classify} and~\ref{sec:ranking}.)



\begin{table*}
\begin{center}
\begin{tabular}{c|c|c}
    historyofrock1-001 &       sustainableag-001 &        molevol-001         \\    
     nuclearscience-001 &       mentalhealth-002         sdn-001           \\
     images-2012-001 &          genchem1-001 &             operations-002       \\  
    macroeconomics-001 &       lyingcamera-001 &          malsoftware-001       \\ 
     ml-003             &      intlcriminallaw-001 &      drugdiscovery-001       \\
     introeulaw-001 &           orgchem2a-001 &            mosfet-001             \\
     pgm-003      &            programming2-001 &         einstein-001          \\
     behavioralecon-001 &       fe-001 &                   rationing-001         \\
     hci-003       &           ancientgreeks-001 &        programming1-2012-001  \\ 
     medicalneuro-001 &         globalfoodsystems-001 &    hollywood-001          \\
     healthforall-002       &  healthinformatics-001 &    lawandecon-001         \\
     rosc-001 &                 programdesign-001 &        nutrition-002          \\
     wealthofnations-001 &      modernpostmodern-001 &     socialepi-001   \\        
     hwswinterface-001 &        intropsych-001 &           art-001                 \\
     adhd-001 &                 digitalmedia-001 &         mythology-002          \\
     engcomlaw-001 &            neuralnets-2012-001 &      analyticalchem-001 \\     
     posa-001 &                 progfun-002       &       crypto-007             \\
     introstats-001 &           datasci-001 &              climateliteracy-001     \\
     gametheory-2012-002      healthpolicy-002  &       lead-ei-001        \\     
     ecfoodandyou-001 &         audiomusicengpart1-001 &   sciwrite-2012-001  \\     
     gtcomp-001 &               friendsmoneybytes-002 &    usefulgenetics-001      \\
     globalenergy-001 &         aboriginaled-001 &         nlangp-001              \\
     compilers-2012-002  &     oldglobe-001 &             networksonline-001  \\   
     secrets-001 &              bluebrain-001 &            newwayhealthcare-001\\   
     bioelectricity-002     
\end{tabular}
\end{center}
\caption{List of courses for statistical analysis}
\label{atab:stat}
\end{table*}


\begin{table*}
\begin{center}
 \begin{tabular}{c|c|c}
    sustainableag-001 &        molevol-001 &              nuclearscience-001      \\
     mentalhealth-002         sdn-001 &                  images-2012-001        \\
    genchem1-001 &             macroeconomics-001 &       malsoftware-001    \\    
    intlcriminallaw-001 &      drugdiscovery-001 &        orgchem2a-001           \\
    mosfet-001 &               pgm-003      &            programming2-001        \\
    einstein-001 &             rationing-001 &            hci-003                \\
    ancientgreeks-001 &        medicalneuro-001 &         globalfoodsystems-001   \\
    healthforall-002    &     healthinformatics-001 &    rosc-001                \\
    programdesign-001 &        wealthofnations-001 &      socialepi-001        \\   
    art-001 &                  digitalmedia-001 &         mythology-002          \\
    engcomlaw-001 &            neuralnets-2012-001 &      analyticalchem-001   \\   
    posa-001 &                 progfun-002         &     crypto-007             \\
    introstats-001 &           climateliteracy-001 &      healthpolicy-002    \\   
    ecfoodandyou-001 &         audiomusicengpart1-001 &   sciwrite-2012-001  \\     
    gtcomp-001 &               friendsmoneybytes-002 &   usefulgenetics-001      \\
    nlangp-001 &               compilers-2012-002    &   oldglobe-001            \\
    networksonline-001 &       secrets-001 &              bioelectricity-002    \\
\end{tabular}
\end{center}
\caption{List of courses that pass the Shapiro tests.}
\label{atab:shapiro}
\end{table*}

\begin{table*}
\begin{center}
\begin{tabular}{c|c|c}
    historyofrock1-001 &       sustainableag-001 &        molevol-001         \\    
     nuclearscience-001 &       mentalhealth-002         sdn-001           \\
     images-2012-001 &          genchem1-001 &             operations-002       \\  
    macroeconomics-001 &       lyingcamera-001 &          malsoftware-001       \\ 
     ml-003             &      intlcriminallaw-001 &      drugdiscovery-001       \\
     introeulaw-001 &           orgchem2a-001 &            mosfet-001             \\
     pgm-003      &            programming2-001 &         einstein-001          \\
     behavioralecon-001 &       fe-001 &                   rationing-001         \\
     hci-003       &           ancientgreeks-001 &        programming1-2012-001  \\ 
     medicalneuro-001 &         globalfoodsystems-001 &    hollywood-001          \\
     healthforall-002       &  healthinformatics-001 &    lawandecon-001         \\
     rosc-001 &                 programdesign-001 &        nutrition-002          \\
     wealthofnations-001 &      modernpostmodern-001 &     socialepi-001   \\        
     hwswinterface-001 &        intropsych-001 &           art-001                 \\
     adhd-001 &                 digitalmedia-001 &         mythology-002          \\
     engcomlaw-001 &            neuralnets-2012-001 &      analyticalchem-001 \\     
     posa-001 &                 progfun-002       &       crypto-007             \\
     introstats-001 &           datasci-001 &              climateliteracy-001     \\
     gametheory-2012-002      healthpolicy-002  &       lead-ei-001        \\     
     ecfoodandyou-001 &         audiomusicengpart1-001 &   sciwrite-2012-001  \\     
     gtcomp-001 &               friendsmoneybytes-002 &    usefulgenetics-001      \\
     globalenergy-001 &         aboriginaled-001 &         nlangp-001              \\
     compilers-2012-002  &     oldglobe-001 &             networksonline-001  \\   
     secrets-001 &              bluebrain-001 &            newwayhealthcare-001\\   
     bioelectricity-002    &  latinamericanculture-001 & epigenetics-001 \\
compstrategy-001 & compilers-003& compfinance-004
\end{tabular}
\end{center}
\caption{List of courses for forum analysis}
\label{atab:forum}
\end{table*}





==> a-prelim.tex <==

\section{More on data-collection}
We now further explain how the data are colleted. 
 We registered four users in coursera. Then we used these  users to enroll in all the courses that were available in July, 2013. Each user approximately enrolled in 20 to 30 courses. We coded the courses' properties such as the video length, or whether the course is a quantitative one ourselves. We then crawled the forum content by using these users' credential. One specific problem we encountered were that Coursera uses AJAX to render the webpages, \ie the raw html does not contain content-specific information.To address this problem, we used Selenium (and its Python wrapper) to control a Chrome/Firefox kernel and have these browsers to parse the Javascripts. Working with the kernels of the browsers will slow down the throughput. We crawled 1 to 3 pages per second from the Coursera server. Finally,  we used the beautifulsoap to parse the dataset. 

\section{More on Coursera's statistics.}
\myparab{Enrollment in different courses}
Out of 115,922 students, 102,782 students (88.7\%) enroll in only one course, 9938 students (8.6\%) students enroll in two courses, 2029 (1.8\%) enroll in three courses, 1173 students ($\approx 1\%$) enroll 
in more than three courses. 

\myparab{Video length.} Figure~\ref{fig:vlen}a presents the histogram on the distribution of the video lengths across different courses (and a Gaussian curve with the same mean and variance is added). Figure~\ref{fig:vlen}b presents the breakdown in video length by categories. 


\begin{figure}
\begin{center}
\subfigure[Histograms on the video length]{
\includegraphics[scale=0.3]{vlength_dist}}
\subfigure[the video length by categories]{
\includegraphics[scale=0.3]{box_len}}
\end{center}
\vspace{-.5cm}
\caption{Distribution on the length of the videos.}
\label{fig:vlen}
\end{figure}


==> a-topic.tex <==
\section{Missing generative model results.}

\subsection{Missing results in thread classification.}
Figure~\ref{fig:rocall} shows the ROC curve for our SVM classifier. 


\begin{figure}
\begin{center}
\includegraphics[scale=0.3]{roc_all_data}
\end{center}
\caption{The ROC curve for the support vector machine. }
\label{fig:rocall}
\end{figure}
\subsection{Missing proof}
\begin{proof}[ of Theorem~\ref{thm:topical}] For exposition purpose, let us assume each thread has uniform size and contains $s$ words. 

We shall first show part 2, \ie there exists a seperating plane for smalltalk and non-smalltalk type threads. Let $S_0 = \supp(\calt_0)$ be the support of $\calt_0$. Let $\vec a = (a_1, ..., a_n)$ be a 
binary vector such that $a_i = 1$ if and only if $i \in S_0$. 

Now for any $i$, consider the distributions $\cald_0(i)$ and $\cald_1(i)$. We can see that
$$ \E_{\cald_0}[w \in S_0] = \epsilon + c_0 \epsilon \quad \mbox{ and } \quad \E_{\cald_1}[w \in S_0] = c_0 \epsilon$$
for some constant $c_0$. Thus, for any document $W$ of size $s$, we have
$$\E_{\cald^s_0}[\sum_{w \in W}(w \in S_0)] = s(1+c_0) \epsilon  \mbox{ and }  \E_{\cald^s_0}[\sum_{w \in W}(w \in S)] = c_0s\epsilon.$$
We may set the threshold as $\tau = s(\frac 1 2 + c_0)\epsilon$, \ie for any thread $W$ (in the bag-of-word representation), we classify it as a logistic/smalltalk thread if and only if $aW > \tau$. By using a simple Chernoff bound, we see that 
$$\Pr_{\cald^s_0}[aW \geq \tau] = \Pr_{\cald^s_0}[\sum_{w \in W}(w \in S_0) \geq \tau] \geq 1 - \frac 1 n$$
 and $\Pr_{\cald^s_0}[aW \leq \tau] \geq 1 - \frac 1 n$ when $s\epsilon = \Omega(\log n)$. Thus, this separation plane works well in SVM. 


Next, let us move to prove the first part of the theorem. Here we leverage a quite straightforward intuition to construct the negative examples. When we train the classifier per course, there is insufficient number of 
training data and thus with high probability over the training data that the estimates of the conditional 
probability are over-estimates. On the other hand, when we train the classifier against all the courses, 
the classifier cannot address the fact that $p_i$ are different for different courses. Thus, the Naive Bayes classifier will have use a wrong prior for a number of courses. In these courses, the classifier could perform badly. 

We now formalize this intuition. 
Let us start with the case where we train the classifier
per course. Let us focus on the first course. Here, we set $s_1 = \sqrt n$, $p_1 = c\log n /\sqrt n$ for a suitably large constant, and $b_1 = \frac 1 {p_1}$. Furthermore, we adopt the standard approach to initialize the estimates on the conditional probability, \ie $\epr[w\mid \cald_0] = \epr[w \mid \cald_1] = 1$ for all words $w$. 

We can see that from $b_1$ samples,  with constant probability that we see only $O(1)$ positive threads (\ie smalltalk type threads) sampled from $\cald_0$. In this case, the conditional esimtates in the Naive Bayes classifiers are
$$\epr[w\mid \cald_0] = \Theta(1) \quad \mbox{ and } \quad \epr[w \mid \cald_1] = \Theta(\frac 1 n).$$
Also, we have $\epr[\cald_0] = O(p_1)$. Let $W$ be an arbitrary negative thread.  Recall that $\epr[W \in \cald_i \mid W] = \prod_{w \in W}\epr[w\mid\cald_i]\epr[\cald_i]$, $W$ is classified as positive if and only if 
{\small
$$\sum_{w \in W}\log(\epr[w \mid \cald_0]) + \log \epr[\cald_0] > \sum_{w \in W}\log \epr[w \mid \cald_1] + \log \epr[\cald_1].$$}

We can see that (again from Chernoff bounds) with high probability the left-hand side $= \Theta(-s - \log n)$ while the right-hand side $= \Theta(-s\log n)$. Thus, with constant probability over the training data the Naive classifier will misclassify the negative threads with high probability (over the testing data). 

We now move to the case we train the classifier from threads across all the courses. We need only two courses to construct the negative example. Here, we use the same distributions and parameter for the first course as we did in the per-course-classifier analysis. We now specify the second course. We let $s_2 = n^d$ for a constant $d$ to be decided later and let $p_2 = (1-\frac 1{n^d})$. Under this setting, with high probability we see only a constant number of threads from $\cald_1(2)$. Thus $\epr[\cald_0] = O(1/n^d)$, 
$\epr[w\mid \cald_0]$ are all accurate (within a small multiplicative error) while $\epr[w\mid \cald_1]$ is also statistically close to $\cald_1(1)$ (because we only see a constant number of samples from $\cald_1(2)$). Thus, when $W$ is a negative sample, we have
\begin{eqnarray*}
& & \sum_{w \in W}\log\epr[w\mid \cald_0] + \log \epr[\cald_0]  \\
& & \quad \quad -  \sum_{w \in W}\log\epr[w\mid \cald_0] + \log \epr[\cald_0] \\
&\approx& \Theta(\epsilon \ell) - d\log\frac 1 n < 0,
\end{eqnarray*}
for a sufficiently large $d$. Here ``$\approx$'' refers to the sum of r.v.s concentrates around the right hand side. In other words, with constant probability the classifier fails to work for most of the negative samples. 
\end{proof}


\subsection{Topical algorithm}
 The first rows illustrate the number of words in the top-50 list that appear in the $i + 1$-st day but not in the $i$-th day. 
We can see that the set of top-50 words quickly stablizes (the set difference is at most 2 for most of the courses, execpt for posa-001.)

\begin{figure*}
\begin{center}
\includegraphics[scale=0.2]{ml-003-w}
\includegraphics[scale=0.2]{healthforall-002-w}
\includegraphics[scale=0.2]{posa-001-w}
\includegraphics[scale=0.2]{latinamericanculture-001-w}

\end{center}
\caption{Convergence rate of our algorithm for four courses. From left to right: ml-003, healthforall-002, posa-001, latinamericanculture-001. First row: the set difference. The second row: normalized Kendall-Tau distance.}
\label{fig:topicconverge}
\end{figure*}

\subsection{Updates of HITS algorithm}
We use the following procedure to update our HITS type algorithm in Section~\ref{sec:ranking}. 

\begin{enumerate}
\item Initialization: all the authority nodes have uniform weight. 
\item Iteration: in each round, each hub node's weight is the sum of its neighbor's weight. Then we normalize the hub nodes by the $\ell_2$-norm. Then we repeat the same procedure for the authority nodes. 
\item Stopping criteria: if the $\ell_2$ distances of both the authority weight vector and the hub weight vector is sufficiently small, the algorithm terminates. 
\end{enumerate}



\begin{figure}
\begin{center}
\subfigure[Comparing wt tf-idf]{
\hspace{-.5cm}
\includegraphics[scale=0.34]{comp1}}
%includegraphics[scale=0.33]{comp1-bydayv2}}
\subfigure[Comparing wt HITS]{
\includegraphics[scale=0.34]{comp2}}
%\includegraphics[scale=0.33]{comp2-bydayv2}}
\end{center}
\vspace{-.4cm}
\caption{Evaluating the relavance ranking algorithm}
\label{fig:comp1}
\end{figure}

\subsection{More evaluation results for the ranking algorithm.}


==> courses-b.tex <==

\begin{table}
\begin{center}
 \begin{tabular}{c|c|c}
    sustainableag-001 &        molevol-001 &              nuclearscience-001      \\
     mentalhealth-002         sdn-001 &                  images-2012-001        \\
    genchem1-001 &             macroeconomics-001 &       malsoftware-001    \\    
    intlcriminallaw-001 &      drugdiscovery-001 &        orgchem2a-001           \\
    mosfet-001 &               pgm-003      &            programming2-001        \\
    einstein-001 &             rationing-001 &            hci-003                \\
    ancientgreeks-001 &        medicalneuro-001 &         globalfoodsystems-001   \\
    healthforall-002    &     healthinformatics-001 &    rosc-001                \\
    programdesign-001 &        wealthofnations-001 &      socialepi-001        \\   
    art-001 &                  digitalmedia-001 &         mythology-002          \\
    engcomlaw-001 &            neuralnets-2012-001 &      analyticalchem-001   \\   
    posa-001 &                 progfun-002         &     crypto-007             \\
    introstats-001 &           climateliteracy-001 &      healthpolicy-002    \\   
    ecfoodandyou-001 &         audiomusicengpart1-001 &   sciwrite-2012-001  \\     
    gtcomp-001 &               friendsmoneybytes-002 &   usefulgenetics-001      \\
    nlangp-001 &               compilers-2012-002    &   oldglobe-001            \\
    networksonline-001 &       secrets-001 &              bioelectricity-002    \\
\end{tabular}
\end{center}
\caption{List of courses that pass the Shapiro tests.}
\end{table}

==> r_model1.tex <==
\begin{table}
\begin{center}
\begin{tabular}{l D{.}{.}{4.5} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} \\
\midrule
(Intercept) & 18.28         \\
            & (24.70)       \\
$Q_it$         & 1.51^{***}    \\
            & (0.27)        \\
$V_it$         & 3.33^{***}    \\
            & (0.32)        \\
$L_it$        & -0.07^{***}   \\
            & (0.02)        \\
$D_it$        & 0.03^{***}    \\
            & (0.01)        \\
$P_it$        & -0.63^{**}    \\
            & (0.27)        \\
$S_it$        & -0.17^{**}    \\
            & (0.07)        \\
$H_it$         & 0.00          \\
            & (0.01)        \\
$M_it$        & -0.01^{***}   \\
            & (0.00)        \\
$Q_i$          & -13.98        \\
            & (12.00)       \\
$V_i$          & -135.57^{***} \\
            & (16.13)       \\
$L_i$         & 1.96^{**}     \\
            & (0.77)        \\
$D_i$          & -0.56         \\
            & (0.37)        \\
$P_i$         & 88.29^{***}   \\
            & (11.65)       \\
$t$           & -1.86^{***}   \\
            & (0.61)        \\
$S_i$          & 6.05^{**}     \\
            & (2.83)        \\
$H_i$         & 1.40^{**}     \\
            & (0.54)        \\
$M_i$         & 0.48^{***}    \\
            & (0.01)        \\
\midrule
R$^2$       & 0.56          \\
Adj. R$^2$  & 0.55          \\
Num. obs.   & 5074          \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{2}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\end{center}
\caption{The linear model }
\label{table:model1}
\end{table}

==> r_model2.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l D{.}{.}{4.5} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} \\
\midrule
(Intercept) & 70.25^{***}  \\
            & (10.91)      \\
$Q_it$         & 0.85^{***}   \\
            & (0.12)       \\
$V_it$         & 1.46^{***}   \\
            & (0.14)       \\
$L_it$         & -0.02^{***}  \\
            & (0.01)       \\
$D_it$         & 0.03^{***}   \\
            & (0.00)       \\
$P_it$        & -0.38^{***}  \\
            & (0.12)       \\
$S_it$         & -0.07^{**}   \\
            & (0.03)       \\
$H_it$         & 0.00         \\
            & (0.01)       \\
$M'_it$        & 0.00^{***}   \\
            & (0.00)       \\
$Q_i$         & -23.74^{***} \\
            & (5.29)       \\
$V_i$          & -61.40^{***} \\
            & (7.19)       \\
$L_i$          & -0.05        \\
            & (0.34)       \\
$D_i$          & -0.62^{***}  \\
            & (0.17)       \\
$P_i$          & 32.00^{***}  \\
            & (5.16)       \\
t           & -1.98^{***}  \\
            & (0.27)       \\
$S_i$          & 3.25^{***}   \\
            & (1.26)       \\
$H_i$         & 0.97^{***}   \\
            & (0.24)       \\
$M'_i$         & 0.36^{***}   \\
            & (0.01)       \\
\midrule
R$^2$       & 0.47         \\
Adj. R$^2$  & 0.47         \\
Num. obs.   & 5074         \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{2}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\end{center}
\caption{Statistical models}
\label{table:model2}
\end{table}


==> r_model3.tex <==
\begin{table}
\begin{center}
\begin{tabular}{l D{.}{.}{4.5} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} \\
\midrule
(Intercept) & 4.27^{***}  \\
            & (0.15)      \\
$Q_it$         & 0.01^{***}  \\
            & (0.00)      \\
$V_it$        & 0.01^{**}   \\
            & (0.01)      \\
$D_it$        &    6.286\mathrm{e}-04^{***}\\
            & (0.00)      \\
$P_it$         & 3.045\mme-03      \\
            & (0.00)      \\
$S_it$        & -1.470\mme-03 ^{**}   \\
            & (0.00)      \\
$M'_it$        &  -1.892\mme-05^{**}   \\
            & (0.00)      \\
$Q_i$         & -0.19^{**}  \\
            & (0.07)      \\
$V_i$          & -0.15       \\
            & (0.10)      \\
$D_i$          & -0.01^{***} \\
            & (0.00)      \\
$P_i$          & 0.25^{***}  \\
            & (0.07)      \\
$t$           & -0.07^{***} \\
            & (0.01)      \\
$S_i$          & 0.07^{***}  \\
            & (0.01)      \\
$M'_i$         & 2.941\mme-03 ^{***}  \\
            & (0.00)      \\
\midrule
R$^2$       & 0.53        \\
Adj. R$^2$  & 0.53        \\
Num. obs.   & 1711        \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{2}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\end{center}
\caption{Fitting a log-linear model on a subset of courses.}
\label{table:model3}
\end{table}

\begin{figure}
\begin{center}
\includegraphics[scale=0.4]{qqnormmodel3}
\end{center}
\caption{The q-q plot of the residuals}
\label{fig:residuallm}
\end{figure}

==> rr_model1.tex <==
\begin{table}
\begin{center}
\begin{tabular}{l D{.}{.}{-1} @{}}
\toprule
            & \multicolumn{1}{c}{Linear model} \\
\midrule
(Intercept) & 18.28         \\
$Q_it$         & 1.51^{***}    \\
$V_it$         & 3.33^{***}    \\
$L_it$        & -0.07^{***}   \\
$D_it$        & 0.03^{***}    \\
$P_it$        & -0.63^{**}    \\
$S_it$        & -0.17^{**}    \\
$H_it$         & 0.00          \\
$M_it$        & -0.01^{***}   \\
$Q_i$          & -13.98        \\
$V_i$          & -135.57^{***} \\
$L_i$         & 1.96^{**}     \\
$D_i$          & -0.56         \\
$P_i$         & 88.29^{***}   \\
$t$           & -1.86^{***}   \\
$S_i$          & 6.05^{**}     \\
$H_i$         & 1.40^{**}     \\
$M_i$         & 0.48^{***}    \\
\midrule
R$^2$       & 0.56          \\
Adj. R$^2$  & 0.55          \\
Num. obs.   & 5074          \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{2}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\begin{tabular}{l D{.}{.}{-1} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} \\
\midrule
(Intercept) & 70.25^{***}  \\
$Q_it$         & 0.85^{***}   \\
$V_it$         & 1.46^{***}   \\
$L_it$         & -0.02^{***}  \\
$D_it$         & 0.03^{***}   \\
$P_it$        & -0.38^{***}  \\
$S_it$         & -0.07^{**}   \\
$H_it$         & 0.00         \\
$M'_it$        & 0.00^{***}   \\
$Q_i$         & -23.74^{***} \\
$V_i$          & -61.40^{***} \\
$L_i$          & -0.05        \\
$D_i$          & -0.62^{***}  \\
$P_i$          & 32.00^{***}  \\
t           & -1.98^{***}  \\
$S_i$          & 3.25^{***}   \\
$H_i$         & 0.97^{***}   \\
$M'_i$         & 0.36^{***}   \\
\midrule
R$^2$       & 0.47         \\
Adj. R$^2$  & 0.47         \\
Num. obs.   & 5074         \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{2}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\end{center}
\caption{The linear model }
\label{table:model1}
\end{table}

\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{l D{.}{.}{5.5} @{}D{.}{.}{5.5} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} & \multicolumn{1}{c}{Model 2} \\
\midrule
(Intercept) & 18.276         & 70.252^{***}  \\
            & (24.696)       & (10.905)      \\
qit         & 1.511^{***}    & 0.847^{***}   \\
            & (0.269)        & (0.119)       \\
vit         & 3.328^{***}    & 1.463^{***}   \\
            & (0.322)        & (0.144)       \\
lit         & -0.071^{***}   & -0.024^{***}  \\
            & (0.015)        & (0.007)       \\
dit         & 0.034^{***}    & 0.025^{***}   \\
            & (0.008)        & (0.003)       \\
pit         & -0.631^{**}    & -0.375^{***}  \\
            & (0.268)        & (0.119)       \\
tat         & -0.168^{**}    & -0.067^{**}   \\
            & (0.073)        & (0.033)       \\
hwt         & 0.000          & -0.001        \\
            & (0.012)        & (0.005)       \\
medt        & -0.007^{***}   & -0.005^{***}  \\
            & (0.000)        & (0.000)       \\
qi          & -13.975        & -23.737^{***} \\
            & (11.995)       & (5.285)       \\
vi          & -135.567^{***} & -61.404^{***} \\
            & (16.130)       & (7.187)       \\
li          & 1.960^{**}     & -0.049        \\
            & (0.772)        & (0.341)       \\
di          & -0.561         & -0.624^{***}  \\
            & (0.374)        & (0.166)       \\
pi          & 88.289^{***}   & 32.005^{***}  \\
            & (11.649)       & (5.159)       \\
t           & -1.864^{***}   & -1.980^{***}  \\
            & (0.607)        & (0.267)       \\
ta          & 6.050^{**}     & 3.249^{***}   \\
            & (2.832)        & (1.260)       \\
hw          & 1.398^{**}     & 0.973^{***}   \\
            & (0.543)        & (0.239)       \\
med         & 0.481^{***}    & 0.360^{***}   \\
            & (0.008)        & (0.007)       \\
\midrule
R$^2$       & 0.555          & 0.467         \\
Adj. R$^2$  & 0.554          & 0.465         \\
Num. obs.   & 5074           & 5074          \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{3}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\normalsize
\end{center}
\caption{Statistical models}
\label{table:coefficients}
\end{table}


\begin{table}
\begin{center}
\small
\begin{tabular}{l D{.}{.}{5.5} @{}D{.}{.}{5.5} @{}D{.}{.}{5.5} @{}}
\toprule
            & \multicolumn{1}{c}{On $y_{i,t}$} & \multicolumn{1}{c}{On $z_{i,t}$} & \multicolumn{1}{c}{On $\log(z_{i,t})$} \\
\midrule
(Intercept) & 18.276         & 70.252^{***}  & 4.268^{***}  \\
            & (24.696)       & (10.905)      & (0.155)      \\
qit         & 1.511^{***}    & 0.847^{***}   & 0.014^{***}  \\
            & (0.269)        & (0.119)       & (0.004)      \\
vit         & 3.328^{***}    & 1.463^{***}   & 0.011^{**}   \\
            & (0.322)        & (0.144)       & (0.005)      \\
lit         & -0.071^{***}   & -0.024^{***}  &              \\
            & (0.015)        & (0.007)       &              \\
dit         & 0.034^{***}    & 0.025^{***}   & 0.001^{***}  \\
            & (0.008)        & (0.003)       & (0.000)      \\
pit         & -0.631^{**}    & -0.375^{***}  & 0.003        \\
            & (0.268)        & (0.119)       & (0.004)      \\
tat         & -0.168^{**}    & -0.067^{**}   & -0.001^{**}  \\
            & (0.073)        & (0.033)       & (0.001)      \\
hwt         & 0.000          & -0.001        &              \\
            & (0.012)        & (0.005)       &              \\
medt        & -0.007^{***}   & -0.005^{***}  & 0.000^{**}   \\
            & (0.000)        & (0.000)       & (0.000)      \\
qi          & -13.975        & -23.737^{***} & -0.185^{**}  \\
            & (11.995)       & (5.285)       & (0.073)      \\
vi          & -135.567^{***} & -61.404^{***} & -0.153       \\
            & (16.130)       & (7.187)       & (0.104)      \\
li          & 1.960^{**}     & -0.049        &              \\
            & (0.772)        & (0.341)       &              \\
di          & -0.561         & -0.624^{***}  & -0.010^{***} \\
            & (0.374)        & (0.166)       & (0.003)      \\
pi          & 88.289^{***}   & 32.005^{***}  & 0.247^{***}  \\
            & (11.649)       & (5.159)       & (0.073)      \\
t           & -1.864^{***}   & -1.980^{***}  & -0.071^{***} \\
            & (0.607)        & (0.267)       & (0.008)      \\
ta          & 6.050^{**}     & 3.249^{***}   & 0.074^{***}  \\
            & (2.832)        & (1.260)       & (0.015)      \\
hw          & 1.398^{**}     & 0.973^{***}   &              \\
            & (0.543)        & (0.239)       &              \\
med         & 0.481^{***}    & 0.360^{***}   & 0.003^{***}  \\
            & (0.008)        & (0.007)       & (0.000)      \\
\midrule
R$^2$       & 0.555          & 0.467         & 0.530        \\
Adj. R$^2$  & 0.554          & 0.465         & 0.526        \\
Num. obs.   & 5074           & 5074          & 1711         \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{4}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\normalsize
\end{center}
\caption{Statistical models}
\label{table:coefficients}
\end{table}

\begin{table}
\begin{center}
\small
\begin{tabular}{l D{.}{.}{7.5} @{}D{.}{.}{7.5} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} & \multicolumn{1}{c}{Model 2} \\
\midrule
(Intercept) & 18.27583         & 70.25167^{***}  \\
$Q_it$         & 1.51114^{***}    & 0.84676^{***}   \\
$V_it$         & 3.32752^{***}    & 1.46257^{***}   \\
$L_it$         & -0.07132^{***}   & -0.02422^{***}  \\
$D_it$         & 0.03392^{***}    & 0.02507^{***}   \\
$P_it$         & -0.63133^{**}    & -0.37547^{***}  \\
$S_it$         & -0.16800^{**}    & -0.06744^{**}   \\
$H_it$        & -5e-05.00000     & -0.00098        \\
$M_it$        & -0.00664^{***}   & -0.00473^{***}  \\
$Q_i$         & -13.97516        & -23.73710^{***} \\
$V_i$          & -135.56735^{***} & -61.40397^{***} \\
$L_i$          & 1.96038^{**}     & -0.04850        \\
$D_i$         & -0.56149         & -0.62389^{***}  \\
$P_i$          & 88.28890^{***}   & 32.00480^{***}  \\
$t$           & -1.86394^{***}   & -1.97963^{***}  \\
$S_i$          & 6.04983^{**}     & 3.24905^{***}   \\
$H_i$          & 1.39781^{**}     & 0.97349^{***}   \\
$M_i$         & 0.48051^{***}    & 0.36026^{***}   \\
\midrule
R$^2$       & 0.55548          & 0.46692         \\
Adj. R$^2$  & 0.55399          & 0.46513         \\
Num. obs.   & 5074             & 5074            \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{3}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\normalsize
\end{center}
\caption{Statistical models}
\label{table:coefficients}
\end{table}

==> rr_model2.tex <==

\begin{table}
\begin{center}
\begin{tabular}{l D{.}{.}{4.5} @{}}
\toprule
            & \multicolumn{1}{c}{Model 1} \\
\midrule
(Intercept) & 70.25^{***}  \\
$Q_it$         & 0.85^{***}   \\
$V_it$         & 1.46^{***}   \\
$L_it$         & -0.02^{***}  \\
$D_it$         & 0.03^{***}   \\
$P_it$        & -0.38^{***}  \\
$S_it$         & -0.07^{**}   \\
$H_it$         & 0.00         \\
$M'_it$        & 0.00^{***}   \\
$Q_i$         & -23.74^{***} \\
$V_i$          & -61.40^{***} \\
$L_i$          & -0.05        \\
$D_i$          & -0.62^{***}  \\
$P_i$          & 32.00^{***}  \\
t           & -1.98^{***}  \\
$S_i$          & 3.25^{***}   \\
$H_i$         & 0.97^{***}   \\
$M'_i$         & 0.36^{***}   \\
\midrule
R$^2$       & 0.47         \\
Adj. R$^2$  & 0.47         \\
Num. obs.   & 5074         \\
\bottomrule
\vspace{-2mm}\\
\multicolumn{2}{l}{\textsuperscript{***}$p<0.01$, 
  \textsuperscript{**}$p<0.05$, 
  \textsuperscript{*}$p<0.1$}
\end{tabular}
\end{center}
\caption{Statistical models}
\label{table:model2}
\end{table}

